A Tale of Two Markets: Investigating the Ransomware Payments Economy

Ransomware attacks are among the most severe cyber threats. They have made headlines in recent years by threatening the operation of governments, critical infrastructure, and corporations. Collecting and analyzing ransomware data is an important step towards understanding the spread of ransomware and designing effective defense and mitigation mechanisms. We report on our experience operating Ransomwhere, an open crowdsourced ransomware payment tracker to collect information from victims of ransomware attacks. With Ransomwhere, we have gathered 13.5k ransom payments to more than 87 ransomware criminal actors with total payments of more than $101 million. Leveraging the transparent nature of Bitcoin, the cryptocurrency used for most ransomware payments, we characterize the evolving ransomware criminal structure and ransom laundering strategies. Our analysis shows that there are two parallel ransomware criminal markets: commodity ransomware and Ransomware as a Service (RaaS). We notice that there are striking differences between the two markets in the way that cryptocurrency resources are utilized, revenue per transaction, and ransom laundering efficiency. Although it is relatively easy to identify choke points in commodity ransomware payment activity, it is more difficult to do the same for RaaS.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#

TEX = paper
FIGS = 
PSFIGS = $(FIGS:.pdf=.ps)

all: pdf
ps:  $(TEX).ps
pdf: $(TEX).pdf
dvi: $(TEX).dvi

clean:
	$(RM) *.synctex.gz *.out *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.eps dummy
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

# only need -Ppdf if using CM fonts

paper.pdf: *.tex *.bib Makefile sections/*.tex
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $<

embed: paper.pdf
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -sOutputFile=paper-embedfonts.pdf paper.pdf

# This is for a tool of mine that monitors files for changes via
# inotify and then executes actions. --cpk
notif:
	notif -vv *.tex *.bib make

source:
	# Needed to create bbl file
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make $<
	rm -rf source-to-submit
	mkdir -p source-to-submit
	latexpand --verbose --empty-comments paper.tex > source-to-submit/paper.tex
	cp acmart.cls source-to-submit/
	cp ACM-Reference-Format.bst source-to-submit/
	cp paper.bib source-to-submit/
	cp paper.bbl source-to-submit/
	mkdir -p source-to-submit/figures
	cp $$(egrep '.pdf$$' paper.fls | grep -v paper.pdf | cut -d' ' -f2 | sort -u | egrep '^\.') source-to-submit/figures/
	sed -i -E 's+(.*\\includegraphics.*\{).*/(.*)+\1figures/\2+' source-to-submit/paper.tex
	cp Makefile.minimal source-to-submit/Makefile

arxiv: source
	# Apply arxiv note patch
	patch --no-backup-if-mismatch -p1 source-to-submit/paper.tex < arxiv-note.patch


==> sections/commodity.tex <==
\section{Petty Crime: Commodity Ransomware}
Commodity

\subsection{Average Revenue and Transactions}

\subsection{Locky}


==> sections/discussion.tex <==
\section{Discussion} \todo{@George: first draft; .75 page}

We have shown that commodity ransomware has been overtaken by RaaS in terms of total revenue and per attack. Where cyber criminals as a threat actor weren't a concern for many organizations not so long ago, this is now changed and probably remains. However commodity ransomware hasn't gone extinct. New strains are created frequently, hence the recent rise of ransomware targeting IoT devices. But with attackers currently misusing weakly secured low-cost IoT devices \cite{alrawi2021circle} and generally low ransom demands, this only emphasizes our message. RaaS actors are so successful in terms of revenue because of their persistance to infect specific potentially lucrative targets. When RaaS actors would add IoT to their portfolios, the impact would only become worse.

==> sections/relatedwork.tex <==
\section{Related Work}
Below we will focus on the work of other authors focusing on the use of Bitcoin by ransomware actors, as well as other types of cyber-criminal actors.

Huang et al. have focused on 16 million USD in ransom payments by 19,750 victims. This was when commodity ransomware authors were targeting individual home users.

%https://github.com/PlyTools/awesome-blockchain-papers#news

Several industry sources issue regular reports as well.

==> sections/twomarkets.tex <==
\subsection{Respite: 2018-2019}
No More Ransom

Cite this research, not even half of a total of 78 tools tested against 61 ransomware were effective in decrypting the files. %https://www.sciencedirect.com/science/article/pii/S0167404821002935

Ransomware considered a solved problem

Industry sources claiming steady decline %https://www.cybereason.com/blog/ransomware-wanna-cry-not-petya-boeing-atlanta

